The Role of Recurrency in Image Segmentation for Noisy and Limited Sample Settings

The biological brain has inspired multiple advances in machine learning. However, most state-of-the-art models in computer vision do not operate like the human brain, simply because they are not capable of changing or improving their decisions/outputs based on a deeper analysis. The brain is recurrent, while these models are not. It is therefore relevant to explore what would be the impact of adding recurrent mechanisms to existing state-of-the-art architectures and to answer the question of whether recurrency can improve existing architectures. To this end, we build on a feed-forward segmentation model and explore multiple types of recurrency for image segmentation. We explore self-organizing, relational, and memory retrieval types of recurrency that minimize a specific energy function. In our experiments, we tested these models on artificial and medical imaging data, while analyzing the impact of high levels of noise and few-shot learning settings. Our results do not validate our initial hypothesis that recurrent models should perform better in these settings, suggesting that these recurrent architectures, by themselves, are not sufficient to surpass state-of-the-art feed-forward versions and that additional work needs to be done on the topic.

==> introduction/figures/unet.tex <==
\begin{tikzpicture}

    
    \node (center) at (0,0) {};

    \node [draw, rectangle, fill=red, minimum height=160, minimum width=1, inner sep=0] (0_1_layer) at ($(center)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=160, minimum width=2.5, inner sep=0] (0_2_layer) at ($(0_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=160, minimum width=2.5, inner sep=0] (0_3_layer) at ($(0_2_layer.east)+(0.4,0)$) {};
    
    \node [draw, rectangle, fill=blue, minimum height=80, anchor=north, minimum width=2.5, inner sep=0] (1_1_layer) at ($(0_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=80, minimum width=5, inner sep=0] (1_2_layer) at ($(1_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=80, minimum width=5, inner sep=0] (1_3_layer) at ($(1_2_layer.east)+(0.4,0)$) {};


    \node [draw, rectangle, fill=blue, minimum height=40, anchor=north, minimum width=5, inner sep=0] (2_1_layer) at ($(1_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=40, minimum width=10, inner sep=0] (2_2_layer) at ($(2_1_layer.east)+(0.6,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=40, minimum width=10, inner sep=0] (2_3_layer) at ($(2_2_layer.east)+(0.6,0)$) {};

    \node [draw, rectangle, fill=blue, minimum height=20, anchor=north, minimum width=10, inner sep=0] (3_1_layer) at ($(2_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=20, minimum width=20, inner sep=0] (3_2_layer) at ($(3_1_layer.east)+(0.8,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=20, minimum width=20, inner sep=0] (3_3_layer) at ($(3_2_layer.east)+(0.8,0)$) {};

    
    \node [draw, rectangle, fill=blue, minimum height=10, anchor=north, minimum width=20, inner sep=0] (4_1_layer) at ($(3_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=10, minimum width=40, inner sep=0] (4_2_layer) at ($(4_1_layer.east)+(1.,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=10, minimum width=40, inner sep=0] (4_3_layer) at ($(4_2_layer.east)+(1.,0)$) {};
    %\node [draw, circle, fill=red, minimum size=20, inner sep=0] (1st layer) at ($(center)+(0,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=20, minimum width=20, inner sep=0] (5_0_layer) at ($(4_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=20, minimum width=20, inner sep=0] (5_1_layer) at ($(5_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=20, minimum width=20, inner sep=0] (5_2_layer) at ($(5_1_layer.east)+(0.8,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=20, minimum width=20, inner sep=0] (5_3_layer) at ($(5_2_layer.east)+(0.8,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=40, minimum width=10, inner sep=0] (6_0_layer) at ($(5_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=40, minimum width=10, inner sep=0] (6_1_layer) at ($(6_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=40, minimum width=10, inner sep=0] (6_2_layer) at ($(6_1_layer.east)+(0.6,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=40, minimum width=10, inner sep=0] (6_3_layer) at ($(6_2_layer.east)+(0.6,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=80, minimum width=5, inner sep=0] (7_0_layer) at ($(6_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=80, minimum width=5, inner sep=0] (7_1_layer) at ($(7_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=80, minimum width=5, inner sep=0] (7_2_layer) at ($(7_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=80, minimum width=5, inner sep=0] (7_3_layer) at ($(7_2_layer.east)+(0.4,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=160, minimum width=2.5, inner sep=0] (8_0_layer) at ($(7_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=160, minimum width=2.5, inner sep=0] (8_1_layer) at ($(8_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=160, minimum width=2.5, inner sep=0] (8_2_layer) at ($(8_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=green, minimum height=160, minimum width=2.5, inner sep=0] (8_3_layer) at ($(8_2_layer.east)+(0.4,0)$) {};

    \draw[->, line width=3] ($(0_3_layer.east)+(0.2,0)$) -- ($(8_0_layer.west)+(-0.2,0)$);
    \draw[->, line width=3] ($(1_3_layer.east)+(0.2,0)$) -- ($(7_0_layer.west)+(-0.2,0)$);
    \draw[->, line width=3] ($(2_3_layer.east)+(0.2,0)$) -- ($(6_0_layer.west)+(-0.2,0)$);
    \draw[->, line width=3] ($(3_3_layer.east)+(0.2,0)$) -- ($(5_0_layer.west)+(-0.2,0)$);

    \draw[->] ($(0_1_layer.east)$) -- ($(0_2_layer.west)$);
    \draw[->] ($(0_2_layer.east)$) -- ($(0_3_layer.west)$);
    \draw[->] ($(1_1_layer.east)$) -- ($(1_2_layer.west)$);
    \draw[->] ($(1_2_layer.east)$) -- ($(1_3_layer.west)$);
    \draw[->] ($(2_1_layer.east)$) -- ($(2_2_layer.west)$);
    \draw[->] ($(2_2_layer.east)$) -- ($(2_3_layer.west)$);
    \draw[->] ($(3_1_layer.east)$) -- ($(3_2_layer.west)$);
    \draw[->] ($(3_2_layer.east)$) -- ($(3_3_layer.west)$);
    \draw[->] ($(4_1_layer.east)$) -- ($(4_2_layer.west)$);
    \draw[->] ($(4_2_layer.east)$) -- ($(4_3_layer.west)$);
    \draw[->] ($(5_1_layer.east)$) -- ($(5_2_layer.west)$);
    \draw[->] ($(5_2_layer.east)$) -- ($(5_3_layer.west)$);
    \draw[->] ($(6_1_layer.east)$) -- ($(6_2_layer.west)$);
    \draw[->] ($(6_2_layer.east)$) -- ($(6_3_layer.west)$);
    \draw[->] ($(7_1_layer.east)$) -- ($(7_2_layer.west)$);
    \draw[->] ($(7_2_layer.east)$) -- ($(7_3_layer.west)$);
    \draw[->] ($(8_1_layer.east)$) -- ($(8_2_layer.west)$);
    \draw[->] ($(8_2_layer.east)$) -- ($(8_3_layer.west)$);

    \draw[->, line width=1] ($(0_3_layer.south)+(0,-0.05)$) -- ($(1_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(1_3_layer.south)+(0,-0.05)$) -- ($(2_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(2_3_layer.south)+(0,-0.05)$) -- ($(3_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(3_3_layer.south)+(0,-0.05)$) -- ($(4_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(4_3_layer.north)+(0,0.05)$) -- ($(5_0_layer.south east)+(0,-0.05)$);
    \draw[->, line width=1] ($(5_3_layer.north)+(0,0.05)$) -- ($(6_0_layer.south east)+(0,-0.05)$);
    \draw[->, line width=1] ($(6_3_layer.north)+(0,0.05)$) -- ($(7_0_layer.south east)+(0,-0.05)$);
    \draw[->, line width=1] ($(7_3_layer.north)+(0,0.05)$) -- ($(8_0_layer.south east)+(0,-0.05)$);
    
\end{tikzpicture}

==> introduction/figures/unet_dynamic.tex <==
\begin{tikzpicture}

    
    \node (center) at (0,0) {};

    \node [draw, rectangle, fill=red, minimum height=160, minimum width=1, inner sep=0] (0_1_layer) at ($(center)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=160, minimum width=2.5, inner sep=0] (0_2_layer) at ($(0_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=160, minimum width=2.5, inner sep=0] (0_3_layer) at ($(0_2_layer.east)+(0.4,0)$) {};
    
    \node [draw, rectangle, fill=blue, minimum height=80, anchor=north, minimum width=2.5, inner sep=0] (1_1_layer) at ($(0_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=80, minimum width=5, inner sep=0] (1_2_layer) at ($(1_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=80, minimum width=5, inner sep=0] (1_3_layer) at ($(1_2_layer.east)+(0.4,0)$) {};


    \node [draw, rectangle, fill=blue, minimum height=40, anchor=north, minimum width=5, inner sep=0] (2_1_layer) at ($(1_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=40, minimum width=10, inner sep=0] (2_2_layer) at ($(2_1_layer.east)+(0.6,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=40, minimum width=10, inner sep=0] (2_3_layer) at ($(2_2_layer.east)+(0.6,0)$) {};

    \node [draw, rectangle, fill=blue, minimum height=20, anchor=north, minimum width=10, inner sep=0] (3_1_layer) at ($(2_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=20, minimum width=20, inner sep=0] (3_2_layer) at ($(3_1_layer.east)+(0.8,0)$) {};
    \node [draw, rectangle, fill=cyan, minimum height=20, minimum width=20, inner sep=0] (3_3_layer) at ($(3_2_layer.east)+(0.8,0)$) {};

    
    \node [draw, rectangle, fill=blue, minimum height=10, anchor=north, minimum width=20, inner sep=0] (4_1_layer) at ($(3_3_layer.south)+(0,-0.5)$) {};
    \node [draw, rectangle, fill=blue, minimum height=10, minimum width=40, inner sep=0] (4_2_layer) at ($(4_1_layer.east)+(1.,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=10, minimum width=40, inner sep=0] (4_3_layer) at ($(4_2_layer.east)+(1.,0)$) {};
    %\node [draw, circle, fill=red, minimum size=20, inner sep=0] (1st layer) at ($(center)+(0,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=20, minimum width=20, inner sep=0] (5_0_layer) at ($(4_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=20, minimum width=20, inner sep=0] (5_1_layer) at ($(5_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=20, minimum width=20, inner sep=0] (5_2_layer) at ($(5_1_layer.east)+(0.8,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=20, minimum width=20, inner sep=0] (5_3_layer) at ($(5_2_layer.east)+(0.8,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=40, minimum width=10, inner sep=0] (6_0_layer) at ($(5_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=40, minimum width=10, inner sep=0] (6_1_layer) at ($(6_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=40, minimum width=10, inner sep=0] (6_2_layer) at ($(6_1_layer.east)+(0.6,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=40, minimum width=10, inner sep=0] (6_3_layer) at ($(6_2_layer.east)+(0.6,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=80, minimum width=5, inner sep=0] (7_0_layer) at ($(6_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=80, minimum width=5, inner sep=0] (7_1_layer) at ($(7_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=80, minimum width=5, inner sep=0] (7_2_layer) at ($(7_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=80, minimum width=5, inner sep=0] (7_3_layer) at ($(7_2_layer.east)+(0.4,0)$) {};

    \node [draw, rectangle, fill=cyan, anchor=south east, minimum height=160, minimum width=2.5, inner sep=0] (8_0_layer) at ($(7_3_layer.north)+(0.0,0.5)$) {};
    \node [draw, rectangle, fill=blue, anchor=west, minimum height=160, minimum width=2.5, inner sep=0] (8_1_layer) at ($(8_0_layer.east)+(0,0)$) {};
    \node [draw, rectangle, fill=blue, minimum height=160, minimum width=2.5, inner sep=0] (8_2_layer) at ($(8_1_layer.east)+(0.4,0)$) {};
    \node [draw, rectangle, fill=green, minimum height=160, minimum width=2.5, inner sep=0] (8_3_layer) at ($(8_2_layer.east)+(0.4,0)$) {};

    \draw[->, line width=3] ($(0_3_layer.east)+(0.2,0)$) -- ($(8_0_layer.west)+(-0.2,0)$);
    \draw[->, line width=3] ($(1_3_layer.east)+(0.2,0)$) -- ($(7_0_layer.west)+(-0.2,0)$);
    \draw[->, line width=3] ($(2_3_layer.east)+(0.2,0)$) -- ($(6_0_layer.west)+(-0.2,0)$);
    \draw[->, line width=3] ($(3_3_layer.east)+(0.2,0)$) -- ($(5_0_layer.west)+(-0.2,0)$);

    \draw[->] ($(0_1_layer.east)$) -- ($(0_2_layer.west)$);
    \draw[->] ($(0_2_layer.east)$) -- ($(0_3_layer.west)$);
    \draw[->] ($(1_1_layer.east)$) -- ($(1_2_layer.west)$);
    \draw[->] ($(1_2_layer.east)$) -- ($(1_3_layer.west)$);
    \draw[->] ($(2_1_layer.east)$) -- ($(2_2_layer.west)$);
    \draw[->] ($(2_2_layer.east)$) -- ($(2_3_layer.west)$);
    \draw[->] ($(3_1_layer.east)$) -- ($(3_2_layer.west)$);
    \draw[->] ($(3_2_layer.east)$) -- ($(3_3_layer.west)$);
    \draw[->] ($(4_1_layer.east)$) -- ($(4_2_layer.west)$);
    \draw[->] ($(4_2_layer.east)$) -- ($(4_3_layer.west)$);
    \draw[->] ($(5_1_layer.east)$) -- ($(5_2_layer.west)$);
    \draw[->] ($(5_2_layer.east)$) -- ($(5_3_layer.west)$);
    \draw[->] ($(6_1_layer.east)$) -- ($(6_2_layer.west)$);
    \draw[->] ($(6_2_layer.east)$) -- ($(6_3_layer.west)$);
    \draw[->] ($(7_1_layer.east)$) -- ($(7_2_layer.west)$);
    \draw[->] ($(7_2_layer.east)$) -- ($(7_3_layer.west)$);
    \draw[->] ($(8_1_layer.east)$) -- ($(8_2_layer.west)$);
    \draw[->] ($(8_2_layer.east)$) -- ($(8_3_layer.west)$);

    \draw[->, line width=1] ($(0_3_layer.south)+(0,-0.05)$) -- ($(1_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(1_3_layer.south)+(0,-0.05)$) -- ($(2_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(2_3_layer.south)+(0,-0.05)$) -- ($(3_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(3_3_layer.south)+(0,-0.05)$) -- ($(4_1_layer.north)+(0,0.05)$);
    \draw[->, line width=1] ($(4_3_layer.north)+(0,0.05)$) -- ($(5_0_layer.south east)+(0,-0.05)$);
    \draw[->, line width=1] ($(5_3_layer.north)+(0,0.05)$) -- ($(6_0_layer.south east)+(0,-0.05)$);
    \draw[->, line width=1] ($(6_3_layer.north)+(0,0.05)$) -- ($(7_0_layer.south east)+(0,-0.05)$);
    \draw[->, line width=1] ($(7_3_layer.north)+(0,0.05)$) -- ($(8_0_layer.south east)+(0,-0.05)$);

    %dynamic
    \draw[->, line width=10, orange] ($(8_3_layer.east)+(0,1)$) .. controls ($(8_3_layer.east)+(5,5)$) and ($(8_3_layer.east)+(5,-5)$) .. ($(8_3_layer.east)+(0,-1)$);

    \draw[->, line width=10, orange] ($(0_1_layer.west)+(0,1)$) .. controls ($(0_1_layer.west)+(-5,5)$) and ($(0_1_layer.west)+(-5,-5)$) .. ($(0_1_layer.west)+(0,-1)$);
\end{tikzpicture}

==> results/som/figures/neuron_response.tex <==
\begin{tikzpicture}

    \node (fig1) at (0,0) {\includegraphics[width=0.45\textwidth]{results/som/figures/som_response_dynamics.pdf}};
    \node (fig2) [anchor=west] at ($(fig1.east)+(0.,0)$) {\includegraphics[width=0.45\textwidth]{results/som/figures/som_response_change_dynamics.pdf}};

    \node (fig1_legend) at ($(fig1.west)+(0.75,2)$) {\large{\textbf{A}}};
    \node (fig2_legend) at ($(fig2.west)+(0.75,2)$) {\large{\textbf{B}}};
\end{tikzpicture}

==> results/som/som.tex <==
\subsection{Self-organizing dynamics explain neuron response}

\begin{figure}[ht]
    \centering
    \input{results/som/figures/neuron_response}
    \caption{Neuron response dynamics under the self-organizing algorithm.}
    \label{fig:som_neuron_response}
\end{figure}
